Complete results for a numerical evaluation of interior point solvers for large-scale optimal power flow problems

Recent advances in open source interior-point optimization methods and power system related software have provided researchers and educators with the necessary platform for simulating and optimizing power networks with unprecedented convenience. Within the Matpower software platform a combination of several different interior point optimization methods are provided and four different optimal power flow (OPF) formulations are recently available: the Polar-Power, Polar-Current, Cartesian-Power, and Cartesian-Current. The robustness and reliability of interior-point methods for different OPF formulations for minimizing the generation cost starting from different initial guesses, for a wide range of networks provided in the Matpower library ranging from 1951 buses to 193000 buses, will be investigated. Performance profiles are presented for iteration counts, overall time, and memory consumption, revealing the most reliable optimization method for the particular metric.

==> MPOPF/fig_AvgTimePerIterTime.tex <==
\newcommand\offone{-8.0ex}
\newcommand\offtwo{-10.5ex}
\newcommand\offthree{-4.5ex}

\begin{tikzpicture}[scale=1.0]

\begin{axis}
[
    width=0.8\columnwidth,
    height=0.3\columnwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar=2pt,
    bar width=4pt,
    %x=1.44cm,
    xmin=3600,
    ymin=1,
    %axis on top,
    ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    width=\columnwidth,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={3600,4320,4800,5760,7200,8760},
    restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(0.35,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},
    ylabel={Time (s)}
]
\addplot[fill=mycolor1]                                          table [x=N, y=AveragePerIter]{data/HYPEROPTGeneMem0Fig5.dat}; \addlegendentry{BELTISTOS}
\addplot[fill=mycolor2, postaction={pattern=horizontal lines}]   table [x=N, y=AveragePerIter]{data/HYPEROPTGeneMem1Fig5.dat}; \addlegendentry{BELTISTOSmem}      
\addplot[fill=mycolor3, postaction={pattern=crosshatch}]         table [x=N, y=AveragePerIter]{data/IPOPTGeneFig5.dat}; \addlegendentry{IPOPT}
\addplot[fill=mycolor4, postaction={pattern=north east lines}]   table [x=N, y=AveragePerIter]{data/MIPSGeneFig5.dat}; \addlegendentry{MIPS}
\addplot[fill=mycolor5, postaction={pattern=north west lines}]   table [x=N, y=AveragePerIter]{data/KNITROGeneFig5.dat}; \addlegendentry{KNITRO}
\end{axis}
\end{tikzpicture}



==> MPOPF/fig_AvgTimePerIterTimeNs_stacked.tex <==
\newcommand\offone{-8.0ex}
\newcommand\offtwo{-10.5ex}
\newcommand\offthree{-4.5ex}

% \definecolor{mycolor1}{HTML}{845EC2}
% \definecolor{mycolor2}{HTML}{D65DB1}
% \definecolor{mycolor3}{HTML}{FFC75F}
% \definecolor{mycolor4}{HTML}{F9F871}
% \definecolor{mycolor5}{HTML}{008F7A}
% \definecolor{mycolor6}{HTML}{0089BA}

\begin{tikzpicture}[scale=1.0]

\pgfplotstableread{
NS	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
10	265.42	6.1	2.43	2.43	1.59	7.69
30	1764.78	11.85	3.42	1.68	2.73	8.5
50	3005.26	22.9	6.14	1.24	5.43	10.26
100	4386.26	24.3	27.08	2.2	26.66	11.25
}\datatableA %case118
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\pgfplotstableread{
NS	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
10	363.41	12.5	12.53	8.84	11.16	46.06
30	3520.83	26.16	14.83	7.62	11.44	45.41
50	7254.52	33.33	27.84	9.88	13.4	46.17
100	30550.61	95.25	64.06	10.53	37.12	53.3
}\datatableB %case1354pegase
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\pgfplotstableread{
NS	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
10 318.76	18.29	26.1	21.05	21.04	97.44
30 4576.47	23.8	30.58	18.9	24.32	103.54
50 8272.5	45.52	31.04	17.2	25.95	105.68
100	2e5	0	59.61	24.59	52.21	108.02
}\datatableC %case2869pegase
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\begin{groupplot}[max space between ticks=15, group style = {group size = 3 by 1, horizontal sep = 20pt}, width=\textwidth, height = 5.0cm]
    \nextgroupplot[ title = {Case 118},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.15,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={10, 30, 50, 100},
    %restrict y to domain*=1:1e6, % Cut off values limit
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3, legend to name = MPOPFgrouplegendNS},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N_s$},
    ylabel={Time (s)} ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-f]\datatableA;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-s]\datatableA;
    %\addlegendentry{BELTISTOS-OPF solve}
    \addlegendentry{\BELTISTOSOPF{}}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    \addplot[forget plot,fill=mycolor2] table [x=NS, y=BELTISTOSmp-f]\datatableA;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=NS, y=BELTISTOSmp-s]\datatableA;
    %\addlegendentry{BELTISTOS-MP solve}
    \addlegendentry{\BELTISTOSMP{}}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-f]\datatableA;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-s]\datatableA;
    %\addlegendentry{BELTISTOS-MPmem solve}
    \addlegendentry{\BELTISTOSMEM{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {1354 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.15,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={10, 30, 50, 100},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N_s$},    %ylabel={Time (s)}
    ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-f]\datatableB;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-s]\datatableB;
    %\addlegendentry{BELTISTOS-OPF solve}
    %\addlegendentry{BELTISTOS-OPF}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor2] table [x=NS, y=BELTISTOSmp-f]\datatableB;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=NS, y=BELTISTOSmp-s]\datatableB;
    %\addlegendentry{BELTISTOS-MP solve}
    %\addlegendentry{BELTISTOS-MP}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-f]\datatableB;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-s]\datatableB;
    %\addlegendentry{BELTISTOS-MPmem solve}
    %\addlegendentry{BELTISTOS-MPmem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {2869 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.15,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={10, 30, 50, 100},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N_s$},    %ylabel={Time (s)}
    ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-f]\datatableC;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=NS, y=BELTISTOSopf-s]\datatableC;
    %\addlegendentry{BELTISTOS-OPF solve}
    %\addlegendentry{BELTISTOS-OPF}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor2] table [x=NS, y=BELTISTOSmp-f]\datatableC;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=NS, y=BELTISTOSmp-s]\datatableC;
    %\addlegendentry{BELTISTOS-MP solve}
    %\addlegendentry{BELTISTOS-MP}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-f]\datatableC;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=NS, y=BELTISTOSmpmem-s]\datatableC;
    %\addlegendentry{BELTISTOS-MPmem solve}
    %\addlegendentry{BELTISTOS-MPmem}    
    
\end{groupplot}
\node at ($(group c2r1) + (0,-3cm)$) {\ref*{MPOPFgrouplegendNS}}; 

\end{tikzpicture}



==> MPOPF/fig_AvgTimePerIterTime_stacked.tex <==
\newcommand\offone{-8.0ex}
\newcommand\offtwo{-10.5ex}
\newcommand\offthree{-4.5ex}

% \definecolor{mycolor1}{HTML}{845EC2}
% \definecolor{mycolor2}{HTML}{D65DB1}
% \definecolor{mycolor3}{HTML}{FFC75F}
% \definecolor{mycolor4}{HTML}{F9F871}
% \definecolor{mycolor5}{HTML}{008F7A}
% \definecolor{mycolor6}{HTML}{0089BA}

\begin{tikzpicture}[scale=1.0]

\pgfplotstableread{
N	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
600	    265.42	2.51	2.43	2.43	1.59	7.69
1200	900.09	21.5	5.38	4.73	3.2	14.81
2400	11136.42	34.83	9.63	9.5	7.69	31.51
4800	1e5	1e5	29.37	23.49	18.97	57.3
}\datatableA %case118
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\pgfplotstableread{
N	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
600	363.41	12.5	12.53	8.84	11.16	46.06
1200	1094.72	20.26	28.15	15.96	18.45	84.59
2400	1.00E+05	1.00E+05	50.63	37.12	41.96	174.86
4800	1.00E+05	1.00E+05	123.78	72.4	82.48	341.97
}\datatableB %case1354pegase
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\pgfplotstableread{
N	BELTISTOSopf-f	BELTISTOSopf-s	BELTISTOSmp-f	BELTISTOSmp-s	BELTISTOSmpmem-f	BELTISTOSmpmem-s
600	518.76	18.29	26.1	21.05	21.04	97.44
1200	1.00E+05	1.00E+05	77.68	38.88	43.59	189.28
2400	1.00E+05	1.00E+05	111.46	95.13	82	368.77
4800	1.00E+05	1.00E+05	225.88	163.42	171.58	760.54
}\datatableC %case2869pegase
%https://docs.google.com/spreadsheets/d/15hEQA_qLJFqDP9tC0Ft9BNeJOkwduImc5wQTJbz8Px0/edit#gid=1528919105

\begin{groupplot}[max space between ticks=15, group style = {group size = 3 by 1, horizontal sep = 20pt}, width=0.9\textwidth, height = 5.0cm]
    \nextgroupplot[ title = {Case 118},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut off values limit
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3, legend to name = MPOPFgrouplegend},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},
    ylabel={Time (s)} ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-f]\datatableA;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-s]\datatableA;
    %\addlegendentry{BELTISTOS-OPF solve}
    \addlegendentry{\BELTISTOSOPF{}}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    \addplot[forget plot,fill=mycolor2] table [x=N, y=BELTISTOSmp-f]\datatableA;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=N, y=BELTISTOSmp-s]\datatableA;
    %\addlegendentry{BELTISTOS-MP solve}
    \addlegendentry{\BELTISTOSMP{}}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-f]\datatableA;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-s]\datatableA;
    %\addlegendentry{BELTISTOS-MPmem solve}
    \addlegendentry{\BELTISTOSMEM{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {1354 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},    %ylabel={Time (s)}
    ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-f]\datatableB;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-s]\datatableB;
    %\addlegendentry{BELTISTOS-OPF solve}
    %\addlegendentry{BELTISTOS-OPF}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor2] table [x=N, y=BELTISTOSmp-f]\datatableB;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=N, y=BELTISTOSmp-s]\datatableB;
    %\addlegendentry{BELTISTOS-MP solve}
    %\addlegendentry{BELTISTOS-MP}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-f]\datatableB;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-s]\datatableB;
    %\addlegendentry{BELTISTOS-MPmem solve}
    %\addlegendentry{BELTISTOS-MPmem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {2869 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    ybar stacked,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 1e5,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},    %ylabel={Time (s)}
    ]
    \addplot[forget plot,fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-f]\datatableC;
    %\addlegendentry{BELTISTOS-OPF factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor1, bar shift=-.25cm] table [x=N, y=BELTISTOSopf-s]\datatableC;
    %\addlegendentry{BELTISTOS-OPF solve}
    %\addlegendentry{BELTISTOS-OPF}
    
    %this resets the stacking and creates a new bar
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor2] table [x=N, y=BELTISTOSmp-f]\datatableC;
    %\addlegendentry{BELTISTOS-MP factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor2] table [x=N, y=BELTISTOSmp-s]\datatableC;
    %\addlegendentry{BELTISTOS-MP solve}
    %\addlegendentry{BELTISTOS-MP}
    
    %this resets the stacking and creates a new bar (which we need to manually shift
    %https://tex.stackexchange.com/questions/13627/pgfplots-multiple-shifted-stacked-plots-in-one-diagram
    \makeatletter
    \pgfplots@stacked@isfirstplottrue
    \makeatother
    
    
    \addplot[forget plot,fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-f]\datatableC;
    %\addlegendentry{BELTISTOS-MPmem factorize} %we forget plot, not included in the legend
    \addplot[fill=mycolor3, bar shift=.25cm] table [x=N, y=BELTISTOSmpmem-s]\datatableC;
    %\addlegendentry{BELTISTOS-MPmem solve}
    %\addlegendentry{BELTISTOS-MPmem}    
    
\end{groupplot}
\node at ($(group c2r1) + (0,-2.8cm)$) {\ref*{MPOPFgrouplegend}}; 

\end{tikzpicture}



==> MPOPF/fig_memory.tex <==
\newcommand\offone{-8.0ex}
\newcommand\offtwo{-10.5ex}
\newcommand\offthree{-4.5ex}

% \definecolor{mycolor1}{HTML}{845EC2}
% \definecolor{mycolor2}{HTML}{D65DB1}
% \definecolor{mycolor3}{HTML}{FFC75F}
% \definecolor{mycolor4}{HTML}{F9F871}
% \definecolor{mycolor5}{HTML}{008F7A}
% \definecolor{mycolor6}{HTML}{0089BA}

\begin{tikzpicture}[scale=1.0]

\pgfplotstableread{
N	OPF	MPOPF	MPOPFmem
600	4050.191406	750.9659082	85.2627832
1200	10292.804688	1501.934072	169.4340723
2400	35070.82031	3003.87041	337.7766602
4800	4e6	6007.743096	674.4618457
}\datatableA %case118
%tampered OPF memory data, the OPF benchmarks were
%run with different binary than the MPOPF bench, furthermore, in OPF we use /usr/bin/time while in MPOPF benchmarks we use beltistos internal memory report

\pgfplotstableread{
N	OPF	MPOPF	MPOPFmem
600	66081.78516	7416.937832	834.3616602
1200	108758.82031	14833.8789	1657.748037
2400	4e6	29667.76104	3304.520801
4800	4e6	59335.52532	6598.066338
}\datatableB %case1354pegase
%tampered OPF memory data, the OPF benchmarks were
%run with different binary than the MPOPF bench, furthermore, in OPF we use /usr/bin/time while in MPOPF benchmarks we use beltistos internal memory report

\pgfplotstableread{
N	OPF	MPOPF	MPOPFmem
600	107606.19531	16751.9172	1872.257041
1200	4e6	33503.84057	3719.688223
2400	4e6	67017.06328	7414.550586
4800	4e6	134034.1318	14804.27532
}\datatableC %case2869pegase
%tampered OPF memory data, the OPF benchmarks were
%run with different binary than the MPOPF bench, furthermore, in OPF we use /usr/bin/time while in MPOPF benchmarks we use beltistos internal memory report

\begin{groupplot}[max space between ticks=15, group style = {group size = 3 by 1, horizontal sep = 20pt}, width=\textwidth, height = 5.0cm]
    \nextgroupplot[ title = {Case 118},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    %ybar stacked,
    ybar,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 2e6,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut off values limit
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.25)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3, legend to name = MPOPFgrouplegend},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},
    ylabel={Memory (MB)} ]
    
    \addplot[fill=mycolor1] table [x=N, y=OPF]\datatableA;
    \addlegendentry{\BELTISTOSOPF{}}
    
    \addplot[fill=mycolor2] table [x=N, y=MPOPF]\datatableA;
    \addlegendentry{\BELTISTOSMP{}}
    
    \addplot[fill=mycolor3] table [x=N, y=MPOPFmem]\datatableA;
    \addlegendentry{\BELTISTOSMEM{}}
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {1354 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    %ybar stacked,
    ybar,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 2e6,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},    %ylabel={Time (s)}
    ]
    \addplot[fill=mycolor1] table [x=N, y=OPF]\datatableB;
    %\addlegendentry{BELTISTOS-OPF}
    
    \addplot[fill=mycolor2] table [x=N, y=MPOPF]\datatableB;
    %\addlegendentry{BELTISTOS-MP}
    
    \addplot[fill=mycolor3] table [x=N, y=MPOPFmem]\datatableB;
    %\addlegendentry{BELTISTOS-MPmem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \nextgroupplot[ title = {2869 Pegase},
    width=0.38\textwidth,
    height=0.3\textwidth,
    separate axis lines,
    %y axis line style= { draw opacity=0 },
    ymajorgrids,
    yminorgrids,
    minor tick num=1,
    %every major grid/.style={black, opacity=1.0},
    %every minor grid/.style={black, opacity=1.0},
    thick,
    every axis plot post/.style={/pgf/number format/fixed},
    %ybar stacked,
    ybar,
    bar width=4pt,
    %x=1.44cm,
    %xmin=3600,
    ymin=1,
    ymax = 2e6,
    %axis on top,
    %ymax=1e6,
    %xtick=data,
    xtick=data,
    ymode=log,
    log basis y=10,
    yminorticks=true,
    enlarge x limits=0.1,
    separate axis lines,
    every outer x axis line/.append style={black},
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    symbolic x coords={600,	1200,	2400,	4800},
    %restrict y to domain*=1:1e6, % Cut values off at 14
    visualization depends on=rawy\as\rawy, % Save the unclipped values
    after end axis/.code={ % Draw line indicating break
            \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.01) -- (rel axis cs:1,1.01);
        },
    axis lines*=left,
    clip=false,
    axis background/.style={fill=none},
    legend style={at={(1.0,1.15)},legend cell align=left,align=left,draw=none,fill=none,font=\scriptsize,legend columns=3},
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},    %ylabel={Time (s)}
    ]
    \addplot[fill=mycolor1] table [x=N, y=OPF]\datatableC;
    %\addlegendentry{BELTISTOS-OPF}
    
    \addplot[fill=mycolor2] table [x=N, y=MPOPF]\datatableC;
    %\addlegendentry{BELTISTOS-MP}
    
    \addplot[fill=mycolor3] table [x=N, y=MPOPFmem]\datatableC;
    %\addlegendentry{BELTISTOS-MPmem}
    
\end{groupplot}
\node at ($(group c2r1) + (0,-3cm)$) {\ref*{MPOPFgrouplegend}}; 

\end{tikzpicture}



==> MPOPF/fig_regression.tex <==
\pgfplotstableread{
%           N          rows         init            fact             solve           total          iters 
%          240     330738              3.82            81.63             3.74            89.19          24    
%          480     661458             13.00           559.03            13.45           585.48          24    
%         1200    1653618             92.23         10377.93            84.70         10554.86          23    
%         1440    1984338            145.09         14236.00            94.60         14475.68          23    
%         2400    3307218            888.34         55715.69           244.94         56848.98          23    
%         2880    3968658            915.55        122752.94           352.77        124021.26          23    
          N              init             fact            solve         total          iters
         240             3.82            81.63             3.74            89.19          24
         480            13.00           559.03            13.45           585.48          24
         720            23.16          1863.58            23.65          1910.39          23
         960            60.36         10645.10            98.66         10804.12          23
        1440           145.09         14236.00            94.60         14475.68          23
        1680           422.38         43937.61           248.78         44608.78          23
        1920           315.52         50905.39           279.59         51500.50          23
        2160          1422.75         59981.01           304.86         61708.62          23
        2880           915.55        122752.94           352.77        124021.26          23
}\datatableIPOPT

    \pgfplotstablecreatecol[ create col/expr={\thisrow{fact}/\thisrow{iters}} ]{factIPOPT}{\datatableIPOPT}
    \pgfplotstablecreatecol[ create col/expr={\thisrow{solve}/\thisrow{iters}} ]{solveIPOPT}{\datatableIPOPT}


\pgfplotstableread{
%          N       rows               init             fact             solve           total          iters
%          240      330738             3.67             6.57             4.05            14.29          24     
%          480      661458             7.34            12.15             7.19            26.68          24   
%         1200     1653618            16.73            32.78            16.73            66.25          23   
%         1440     1984338            22.06            43.22            22.37            87.65          23   
%         2400     3307218            36.86            85.17            37.89           159.92          23   
%         2880     3968658            41.78           107.31            45.76           194.85          23   
%         3600     4960818            51.02           154.23            60.66           265.91          23   
%         4320     5952978            61.70           197.08            71.88           330.66          23   
%         4800     6614418            75.06           237.95            81.75           394.77          23   
%         5760     7937298            92.64           316.50           100.66           509.80          22   
%         7200     9921618           120.01           479.85           138.49           738.34          23   
%         8760    12071298           138.61           682.72           188.25          1009.58          23   
  N        rows              init             fact             solve           total            factPard         factBLU          solvePard      iters        MEMORY
% 240      330738             2.18             0.54             0.28             3.00             0.44             0.03             0.28            1          306.79
% 480      661458             4.23             1.38             0.61             6.22             1.19             0.06             0.60            1          613.58
%  1200     1653618            11.74             3.50             1.28            16.52             2.39             0.28             1.26            1        1533.95
%   1440     1984338            14.06             4.05             1.51            19.62             2.78             0.37             1.49            1        1840.74
%   2400     3307218            24.11             8.63             3.41            36.15             4.87             1.06             3.37            1        3067.91
%   2880     3968658            29.41            10.92             4.46            44.79             6.04             1.51             4.41            1        3681.49
%   3600     4960818            38.09            14.45             5.23            57.77             7.34             2.10             5.17            1        4601.87
%   4320     5952978            44.38            17.43             4.52            66.33             7.80             2.98             4.46            1        5522.24
%   4800     6614418            50.24            21.34             6.65            78.23             9.53             3.67             6.58            1        6135.82
%   5760     7937298            60.33            28.46             6.75            95.55            10.79             5.27             6.68            1        7362.99
%   7200     9921618            75.11            39.39             8.69           123.20            12.86             8.17             8.60            1        9203.74
%   8760    12071298           101.21            61.19            14.79           177.18            17.27            12.78            14.64            1       11197.88
%   9600    13228818            94.04            63.81            12.68           170.53            14.92            14.83            12.54            1       12271.65
%  12000    16536018           130.75           101.75            18.12           250.62            24.32            22.59            17.96            1       15339.56
%  14400    19843218           155.76           142.68            26.14           324.57            28.59            33.80            25.93            1       18407.48
%  17520    24142578           218.97           202.05            30.15           451.17            29.39            50.90            29.80            1        22395.77
%  19200    26457618           232.82           239.18            41.71           513.71            38.38            57.76            41.43            1        24543.31
% 21600    29764818           292.56           323.16            49.83           665.55            42.13            82.69            49.43            1         27611.22
%   240      330738             3.43             0.41             0.26             4.10             0.34             0.02             0.25            1         287.57
%   480      661458             7.48             0.94             0.52             8.94             0.71             0.06             0.51            1         575.14
%  1200     1653618            19.57             2.67             1.11            23.36             1.73             0.26             1.10            1        1437.86
  1440     1984338            23.49             4.09             1.98            29.56             2.50             0.41             1.96            1        1725.43
  2400     3307218            65.68             7.87             2.75            76.30             4.03             1.02             2.71            1        2875.72
  2880     3968658            50.28             9.66             2.88            62.82             5.09             1.39             2.84            1        3450.87
  3600     4960818            62.35            13.05             4.37            79.76             6.11             2.13             4.32            1        4313.59
  4320     5952978            81.62            17.77             6.94           106.33             7.23             3.10             6.87            1        5176.30
  4800     6614418            84.78            21.92             6.02           112.72             9.62             4.06             5.95            1        5751.45
  5760     7937298           101.13            25.94             6.14           133.21             9.46             5.24             6.07            1        6901.74
  7200     9921618           130.41            40.82            11.10           182.32            12.72             8.34            10.99            1        8627.17
  8760    12071298           162.58            63.13            14.31           240.02            15.53            12.15            14.19            1       10496.40
  9600    13228818           177.75            68.27            16.45           262.46            16.73            14.58            16.32            1       11502.90
 12000    16536018           240.64           101.43            18.58           360.65            21.41            24.36            18.39            1       14378.63
 14400    19843218           268.34           133.60            21.38           423.32            25.79            32.11            21.20            1       17254.35
 17520    24142578           342.27           186.62            25.18           554.07            27.54            46.97            24.97            1       20992.80
 19200    26457618           436.19           239.98            40.20           716.38            33.06            57.84            39.74            1       23005.81
 21600    29764818           456.44           323.70            49.57           829.71            43.53            76.86            48.91            1       25881.53
 24000    33072018           588.48           423.26            46.15          1057.88            49.35           111.41            45.63            1       28757.26
}\datatableMPFOPT

    \pgfplotstablecreatecol[ create col/expr={\thisrow{fact}/\thisrow{iters}} ]{factMPFOPT}{\datatableMPFOPT}
    \pgfplotstablecreatecol[ create col/expr={\thisrow{solve}/\thisrow{iters}} ]{solveMPFOPT}{\datatableMPFOPT}
\begin{tikzpicture}
    \pgfplotsset{width=1\columnwidth, height=5cm, legend style={font=\scriptsize}}
    \begin{loglogaxis}[
    every x tick label/.append style={font=\scriptsize},
    every y tick label/.append style={font=\scriptsize},
    ymajorgrids,
    xmajorgrids,
    ytick={1e-1, 1e0, 1e1, 1e2,1e3, 1e4},
    xmin=100,
    yminorgrids,
    xlabel/.append style={font=\scriptsize},
    ylabel/.append style={font=\scriptsize},
    xlabel={$N$},
    ylabel={Time (s)},
    legend cell align=left,
    legend pos=north west]
    \addplot[color=mycolor1,mark size=2.0pt,mark options={fill=mycolor1},only marks] table[x=N,y=factIPOPT]{\datatableIPOPT};
    \label{p1}
    %\addlegendentry{IPOPT factorize}
    
    \addplot[solid,color=mycolor1,line width=1.pt,mark=none] table[x=N,
    y={create col/linear regression={y=factIPOPT}}]{\datatableIPOPT}; % compute a linear regression from the
    \label{p2}

    \xdef\slopeA{\pgfplotstableregressiona} %<-- might be handy occasionally
    \xdef\interceptA{\pgfplotstableregressionb}
    %\addlegendentry{% $\pgfmathprintnumber{\slopeA} \cdot N \pgfmathprintnumber[print sign]{\interceptA}$} %



    \addplot[color=mycolor2,mark size=2.0pt,mark=triangle*,mark options={fill=mycolor2},only marks] table[x=N,y=solveIPOPT]{\datatableIPOPT};
    \label{p3}
    %\addlegendentry{IPOPT solve}
    
    \addplot[dotted,color=mycolor2,line width=1.pt,mark=none] table[x=N,
    y={create col/linear regression={y=solveIPOPT}}]{\datatableIPOPT}; % compute a linear regression from the
    \label{p4}

    \xdef\slopeB{\pgfplotstableregressiona} %<-- might be handy occasionally
    \xdef\interceptB{\pgfplotstableregressionb}

    %\addlegendentry{ $\pgfmathprintnumber{\slopeB} \cdot N \pgfmathprintnumber[print sign]{\interceptB}$} %

      % =================================================================================

    \addplot[color=mycolor4,mark size=2.0pt,mark=square*,mark options={fill=mycolor3},only marks] table[x=N,y=factMPFOPT]{\datatableMPFOPT};
    %\addlegendentry{MPFOPT factorize}
    \label{p5}
    
    \addplot[dashed,color=mycolor4,line width=1.pt,mark=none] table[x=N,
    y={create col/linear regression={y=factMPFOPT}}]{\datatableMPFOPT}; % compute a linear regression from the
    \label{p6}

    \xdef\slopeMPFOPTA{\pgfplotstableregressiona} %<-- might be handy occasionally
    \xdef\interceptMPFOPTA{\pgfplotstableregressionb}
    %\addlegendentry{ $\pgfmathprintnumber{\slopeMPFOPTA} \cdot N \pgfmathprintnumber[print sign]{\interceptMPFOPTA}$} %



    \addplot[color=mycolor5,mark size=2.0pt,mark=diamond*,mark options={fill=mycolor4},only marks] table[x=N,y=solveMPFOPT]{\datatableMPFOPT};
%    \addlegendentry{MPFOPT solve}
    \label{p7}
    
    \addplot[dashdotted,color=mycolor5,line width=1.pt,mark=none] table[x=N,
    y={create col/linear regression={y=solveMPFOPT}}]{\datatableMPFOPT}; % compute a linear regression from the
    \label{p8}

    \xdef\slopeMPFOPTB{\pgfplotstableregressiona} %<-- might be handy occasionally
    \xdef\interceptMPFOPTB{\pgfplotstableregressionb}

%    \addlegendentry{ $\pgfmathprintnumber{\slopeMPFOPTB} \cdot N \pgfmathprintnumber[print sign]{\interceptMPFOPTB}$} %


    \end{loglogaxis}
    \node [draw,fill=white,mark=none,font=\tiny] at (rel axis cs: -0.6,1.01) {\shortstack[l]{
        \ref{p1} BELTISTOS-OPF fact. \\
        \ref{p2} $N^{\pgfmathprintnumber{\slopeA}}$ \\ % \cdot N \pgfmathprintnumber[print sign]{\interceptA}$ \\
        \ref{p3} BELTISTOS-OPF solve \\
        \ref{p4} $N^{\pgfmathprintnumber{\slopeB}}$}}; % \cdot N \pgfmathprintnumber[print sign]{\interceptB}$}};

    \node [draw,fill=white,font=\tiny] at (rel axis cs: 0.1,0.41) {\shortstack[l]{
        \ref{p5} BELTISTOS-MP fact. \\
        \ref{p6} $N^{\pgfmathprintnumber{\slopeMPFOPTA}}$\\ % \cdot N \pgfmathprintnumber[print sign]{\interceptMPFOPTA}$ \\
        \ref{p7} BELTISTOS-MP solve \\
        \ref{p8} $N^{\pgfmathprintnumber{\slopeMPFOPTB}}$}}; % \cdot N \pgfmathprintnumber[print sign]{\interceptMPFOPTB}$}};

  
\end{tikzpicture}



==> OPFbenchmarks_old.tex <==
\pgfplotstableread{
case MIPS MIPSsc FMINCON IPOPT
case1951rte 4.25 4.19 19.18 3.68
case2383wp 4.78 5.53 65.26 6.73
case2736sp 4.63 5.47 15.81 3.45
case2737sop 4.60 5.56 11.02 3.60
case2746wop 5.41 6.23 14.17 4.12
case2746wp 5.06 6.04 14.97 3.66
case2868rte 4.79 5.37 38.50 5.01
case2869pegase 5.53 7.05 11.13 8.29
case3012wp 5.36 6.72 NaN 8.88
case3120sp 6.35 7.27 19.85 8.07
case3375wp 5.96 6.91 NaN 8.30
case6468rte 11.63 13.78 NaN 7.25
case6470rte 13.26 16.13 86.82 9.33
case6495rte 20.51 25.51 35.33 9.46
case6515rte 15.83 19.15 79.59 8.92
case9241pegase 21.00 25.50 194.47 30.32
case\_ACTIVSg2000 4.88 5.40 9.76 3.60
case\_ACTIVSg10k 38.96 55.98 60.74 12.92
case\_ACTIVSg25k 91.92 125.25 261.47 43.80
case\_ACTIVSg70k NaN NaN 874.61 1719.07
case13659pegase NaN 35.94 2816.99 16.22
case21k 141.98 152.41 1915.09 58.22
case42k 606.47 644.25 NaN 183.74
case99k 8853.59 8978.73 20328.19 747.39
case193k NaN NaN NaN 3561.44
}\OPFtabletime

\pgfplotstableread{
case MIPS MIPSsc FMINCON IPOPT
case1951rte 26.00 26.00 62.00 28.00
case2383wp 30.00 31.00 85.00 30.00
case2736sp 27.00 27.00 44.00 20.00
case2737sop 25.00 25.00 31.00 22.00
case2746wop 29.00 28.00 39.00 29.00
case2746wp 28.00 28.00 41.00 23.00
case2868rte 26.00 26.00 60.00 33.00
case2869pegase 28.00 29.00 28.00 29.00
case3012wp 29.00 29.00 NaN 38.00
case3120sp 33.00 33.00 52.00 33.00
case3375wp 30.00 30.00 NaN 33.00
case6468rte 38.00 39.00 NaN 32.00
case6470rte 42.00 44.00 45.00 44.00
case6495rte 69.00 67.00 47.00 50.00
case6515rte 52.00 51.00 74.00 45.00
case9241pegase 40.00 41.00 44.00 39.00
case\_ACTIVSg2000 30.00 28.00 26.00 21.00
case\_ACTIVSg10k 78.00 80.00 52.00 31.00
case\_ACTIVSg25k 69.00 73.00 48.00 42.00
case\_ACTIVSg70k NaN NaN 79.00 265.00
case13659pegase NaN 50.00 63.00 50.00
case21k 49.00 49.00 375.00 48.00
case42k 59.00 59.00 NaN 52.00
case99k 73.00 73.00 358.00 61.00
case193k NaN NaN NaN 76.00
}\OPFtableiters

\pgfplotstableread{
case MIPS MIPSsc FMINCON IPOPT
case1951rte 461.46 463.86 524.11 459.86
case2383wp 481.42 497.93 544.34 487.20
case2736sp 488.13 500.05 544.45 474.72
case2737sop 491.52 489.15 532.84 494.90
case2746wop 488.50 484.18 539.09 480.17
case2746wp 508.53 493.25 571.81 473.05
case2868rte 482.64 479.11 550.85 479.73
case2869pegase 492.66 507.09 549.28 490.68
case3012wp 488.91 495.01 NaN 478.42
case3120sp 493.13 490.98 561.11 479.32
case3375wp 508.26 511.25 NaN 482.41
case6468rte 589.54 598.60 NaN 535.70
case6470rte 594.53 625.32 656.67 547.27
case6495rte 598.50 624.71 652.51 536.77
case6515rte 604.40 620.07 652.33 540.36
case9241pegase 648.16 657.04 809.98 604.31
case\_ACTIVSg2000 482.42 503.54 554.42 473.17
case\_ACTIVSg10k 711.12 702.07 835.14 638.29
case\_ACTIVSg25k 1059.73 1090.79 1428.25 1016.62
case\_ACTIVSg70k NaN NaN 2858.47 2047.15
case13659pegase NaN 786.38 953.72 644.91
case21k 1798.14 1797.71 1919.46 1213.91
case42k 4626.07 4619.28 NaN 2074.63
case99k 22034.14 22127.15 9524.23 4356.91
case193k NaN NaN NaN 8088.29
}\OPFtablememory

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
	\centering
	\caption{Time to solution in seconds of the OPF benchmarks using PF solution as initial guess and Polar-Power formulation\label{tab:OPFsummary-t}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
	precision=1, fixed zerofill, column type={r},
	columns/Statistic/.style={string type,column type=l},
	every row/.style={
		column type=r,
		dec sep align,
		fixed,
		fixed zerofill,
	},
	columns={case,MIPS,MIPSsc,FMINCON,IPOPT},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	columns/case/.style={string type, column type={l}, column name={Benchmark}},
	]\OPFtabletime
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
	\centering
	\caption{Iterations until convergence of the OPF benchmarks using PF solution as initial guess and Polar-Power formulation\label{tab:OPFsummary-i}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
	precision=0, fixed zerofill, column type={r},
	columns/Statistic/.style={string type,column type=l},
	every row/.style={
		column type=r,
		dec sep align,
		fixed,
		fixed zerofill,
	},
	columns={case,MIPS,MIPSsc,FMINCON,IPOPT},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	columns/case/.style={string type, column type={l}, column name={Benchmark}},
	]\OPFtableiters
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
	\centering
	\caption{Memory requirements in kB of the OPF benchmarks using PF solution as initial guess and Polar-Power formulation\label{tab:OPFsummary-m}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
	precision=1, fixed zerofill, column type={r},
	columns/Statistic/.style={string type,column type=l},
	every row/.style={
		column type=r,
		dec sep align,
		fixed,
		fixed zerofill,
	},
	columns={case,MIPS,MIPSsc,FMINCON,IPOPT},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	columns/case/.style={string type, column type={l}, column name={Benchmark}},
	]\OPFtablememory
\end{table}

==> OPFvariantsMIPS.tex <==
\pgfplotstableread{
case polarPower cartPower polarCurrent cartCurrent 
case1951rte          4.4215450000 {} 3.5532190000 4.3991700000
case2383wp           3.7454660000 3.5984240000 3.2128900000 3.9613690000
case2736sp           4.6030680000 3.8816610000 3.0817450000 4.1096720000
case2737sop          4.3193690000 3.3480890000 2.7855480000 3.5674830000
case2746wop          4.2936730000 3.1861140000 2.9533470000 3.5685110000
case2746wp           4.7261540000 3.9079740000 3.1819070000 3.9829600000
case2868rte          4.1577470000 3.9400290000 {} {}
case2869pegase       13.4702450000 8.7076910000 9.3927650000 {}
case3012wp           4.7913490000 4.2725650000 3.8306790000 4.4114910000
case3120sp           17.3509690000 7.3601370000 6.0128020000 6.8722120000
case3375wp           5.6765660000 5.4049530000 4.3984320000 5.2160330000
case6468rte          13.6350410000 {} {} {}
case6470rte          13.2551670000 {} 11.3135920000 {}
case6495rte          {} {} {} {}
case6515rte          16.0727190000 {} 13.6509150000 {}
case9241pegase       40.7093790000 {} 66.3059930000 {}
case\_ACTIVSg2000    4.0439840000 2.9594990000 2.8713640000 2.9569180000
case\_ACTIVSg10k     22.2263710000 25.1226840000 17.9610370000 24.1718050000
case13659pegase      28.9302340000 {} {} {}
case\_ACTIVSg25k     83.5101880000 83.8677280000 69.8420480000 90.6706340000
case\_ACTIVSg70k     {} 334.3281720000 {} {}
case21k               160.5517350000 152.0348090000 129.4009580000 149.1882850000
}\OPFtabletimeMIPS

\pgfplotstableread{
case polarPower cartPower polarCurrent cartCurrent 
case1951rte         26 {} 44 55
case2383wp           29 35 31 38
case2736sp           28 34 27 35
case2737sop          25 30 25 31
case2746wop          25 28 25 30
case2746wp           28 34 28 35
case2868rte          26 33 {} {}
case2869pegase       86 65 73 {}
case3012wp           28 33 29 34
case3120sp           110 53 45 50
case3375wp           30 37 31 37
case6468rte          42 {} {} {}
case6470rte          42 {} 45 {}
case6495rte          {} {} {} {}
case6515rte          53 {} 55 {}
case9241pegase       79 {} 147 {}
case\_ACTIVSg2000    24 27 26 27
case\_ACTIVSg10k     38 55 39 53
case13659pegase      38 {} {} {}
case\_ACTIVSg25k     53 64 57 74
case\_ACTIVSg70k     {} 86 {} {}
case21k               49 57 49 57
}\OPFtableitersMIPS

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
    \footnotesize
	\centering
	\caption{Overall time (s) (\MIPS{} no step control). \label{tab:OPFvariantssummaryMIPS-t}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
	precision=2, fixed zerofill, column type={r},
	columns/Statistic/.style={string type,column type=l},
	every row/.style={
		column type=r,
		dec sep align,
		fixed,
		fixed zerofill,
	},
	columns={case, polarPower, polarCurrent, cartPower, cartCurrent},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	columns/case/.style={string type, column type={l}, column name={Benchmark}},
	columns/polarPower/.style={column name={Polar-Power}},
	columns/polarCurrent/.style={column name={Polar-Current}},
	columns/cartPower/.style={column name={Cartesian-Power}},
	columns/cartCurrent/.style={column name={Cartesian-Current}},
	empty cells with={---} % replace empty cells with ’--’
	]\OPFtabletimeMIPS
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[H]
    \footnotesize
	\centering
	\caption{Number of iterations (\MIPS{} no step control). \label{tab:OPFvariantssummaryMIPS-i}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
	precision=0, fixed zerofill, column type={r},
	columns/Statistic/.style={string type,column type=l},
	every row/.style={
		column type=r,
		dec sep align,
		fixed,
		fixed zerofill,
	},
	columns={case, polarPower, polarCurrent, cartPower, cartCurrent},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	columns/case/.style={string type, column type={l}, column name={Benchmark}},
	columns/polarPower/.style={column name={Polar-Power}},
	columns/polarCurrent/.style={column name={Polar-Current}},
	columns/cartPower/.style={column name={Cartesian-Power}},
	columns/cartCurrent/.style={column name={Cartesian-Current}},
	empty cells with={---} % replace empty cells with ’--’
	]\OPFtableitersMIPS
\end{table}

==> figures/OPFvariantsItersBeltistos.tex <==
\begin{tikzpicture}

% COLORS 
%4-class OrRd Tokyo SIAM PP18
\definecolor{mycolor0}{HTML}{2B83BA}
\definecolor{mycolor1}{HTML}{D7301F}
\definecolor{mycolor2}{HTML}{FC8D59}
\definecolor{mycolor3}{HTML}{FDCC8A}
\definecolor{mycolor4}{HTML}{FEF0D9}
\definecolor{mycolor5}{HTML}{FEF0D9}
\definecolor{mycolor6}{HTML}{009933}

\pgfplotstableread{
id case polarPower cartPower polarCurrent cartCurrent 
1 1951rte      23   16  20  18
2 2383wp       42   45  44  42
3 2736sp       15   22  21  19
4 2737sop      14   15  18  16
5 2746wop      9    17  10  24
6 2746wp       14   27  15  27
7 2868rte      12   20  22  16
8 2869pegase   19   24  20  22
9 3012wp       38   34  38  35
10 3120sp      37   49  35  43
11 3375wp      32   31  39  29
12 6468rte     30   33  34  35
13 6470rte     16   27  17  25
14 6495rte     35   46  37  50
15 6515rte     36   56  51  42
16 9241pegase  33   30  27  46
17 ACTIVSg2000 21   22  21  15
18 ACTIVSg10k  28   15  28  15
19 13659pegase 20   26  30  43
20 ACTIVSg25k  27   36  27  34
21 ACTIVSg70k  33   43  46  27
22 case21k     55   52  54  52
23 case42k     59   62  58  62
24 case99k     71   72  79  72
25 case193k    77   86  81  86
}\itersIPOPT;

\begin{axis}[
width=\columnwidth, height=5.5cm, 
ybar,
bar width=2pt, 
%ymode=log, 
%log origin=infty,
ymin=0,
ymax=250,
axis lines*=left, 
ymajorgrids, yminorgrids,
xtick=data,
xticklabels from table={\itersIPOPT}{case},
%xtick={1,2,3,4,5,6,7,89,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25},
%xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18},
enlarge x limits=0.05,
%xmin=0.5,
%xmax=18.5,
%xticklabels={1, 2, 4, 8, 16, 32, 64, 128, 256},
xticklabel style={align=center, rotate=60, xshift=-0.8cm, yshift=0.2cm, anchor=north, font=\scriptsize},
%ytick={0,20,40,60,80,100},
ytick={0,50,100,150,200,250},
%yticklabels={$10^{-1}$, , , , , , , , $10^0$, , , , , , , , ,$10^1$},
yticklabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
xlabel style={font=\scriptsize},
ylabel={No. of Iterations},
%xlabel={Benchmark},
legend style={at={(1.0,1.05)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=4}
]
\addplot[fill=mycolor0] table[x=id, y=polarPower] {\itersIPOPT};
\addlegendentry{Polar-Power}
\addplot[fill=mycolor1, postaction={pattern=north east lines}] table[x=id, y=cartPower] {\itersIPOPT}; 
\addlegendentry{Cart-Power}
\addplot[fill=mycolor6, postaction={pattern=north west lines}] table[x=id, y=polarCurrent] {\itersIPOPT}; 
\addlegendentry{Polar-Current}
\addplot[fill=mycolor3, postaction={pattern=crosshatch}] table[x=id, y=cartCurrent] {\itersIPOPT}; 
\addlegendentry{Cart-Current}
\end{axis}

\end{tikzpicture}

==> figures/OPFvariantsItersIPOPTdefault.tex <==
\begin{tikzpicture}

% COLORS 
%4-class OrRd Tokyo SIAM PP18
\definecolor{mycolor0}{HTML}{2B83BA}
\definecolor{mycolor1}{HTML}{D7301F}
\definecolor{mycolor2}{HTML}{FC8D59}
\definecolor{mycolor3}{HTML}{FDCC8A}
\definecolor{mycolor4}{HTML}{FEF0D9}
\definecolor{mycolor5}{HTML}{FEF0D9}
\definecolor{mycolor6}{HTML}{009933}

\pgfplotstableread{
id case polarPower cartPower polarCurrent cartCurrent 
1  1951rte 33  33  34  31
2  2383wp  33  35  33  40
3  2736sp  40  27  23  25
4  2737sop 26  27  24  25
5  2746wop 24  18  17  21
6  2746wp  37  26  20  25
7  2868rte 54  44  59  46
8  2869pegase  31  36  45  57
9  3012wp  31  34  31  31
10 3120sp  43  43  47  41
11 3375wp  38  30  270   270
12 6468rte 31  34  34  38
13 6470rte 70  66  81  72
14 6495rte 59  57  52  56
15 6515rte 52  42  46  44
16 9241pegase  44  41  71  79
17 ACTIVSg2000    29  27  28  29
18 ACTIVSg10k 35  34  38  34
19 13659pegase 214 197 193 241
20 ACTIVSg25k 44  46  48  55
21 ACTIVSg70k 83  72  69  76
22 case21k 48  49  270   270
23 case42k 52  54  270   270
24 case99k 62  63  270   270 
25 case193k 77 77 270 270
}\itersIPOPT;
%NAN = 270 (ymax+20)
%11: 38  30  {}   262
%24: 62  63  {}   312

\begin{axis}[
width=\columnwidth, height=5.5cm, 
ybar,
bar width=2pt, 
%ymode=log, 
%log origin=infty,
ymin=0,
ymax=250,
axis lines*=left, 
ymajorgrids, yminorgrids,
xtick=data,
xticklabels from table={\itersIPOPT}{case},
%xtick={1,2,3,4,5,6,7,89,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25},
%xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18},
enlarge x limits=0.05,
%xmin=0.5,
xmax=25,
%xticklabels={1, 2, 4, 8, 16, 32, 64, 128, 256},
xticklabel style={align=center, rotate=60, xshift=-0.8cm, yshift=0.2cm, anchor=north, font=\scriptsize},
ytick={0,50,100,150,200,250},
%yticklabels={$10^{-1}$, , , , , , , , $10^0$, , , , , , , , ,$10^1$},
yticklabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
xlabel style={font=\scriptsize},
ylabel={No. of Iterations},
%xlabel={Benchmark},
legend style={at={(0.3,1.05)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=2},
%restrict y to domain*=250, % Cut values off at 14
% visualization depends on=rawy\as\rawy, % Save the unclipped values
after end axis/.code={ % Draw line indicating break
        \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.02) -- (rel axis cs:1,1.02);
    },
clip=false
]
\addplot[fill=mycolor0] table[x=id, y=polarPower] {\itersIPOPT};
\addlegendentry{Polar-Power}
\addplot[fill=mycolor1, postaction={pattern=north east lines}] table[x=id, y=cartPower] {\itersIPOPT}; 
\addlegendentry{Cart-Power}
\addplot[fill=mycolor6, postaction={pattern=north west lines}] table[x=id, y=polarCurrent] {\itersIPOPT}; 
\addlegendentry{Polar-Current}
\addplot[fill=mycolor3, postaction={pattern=crosshatch}] table[x=id, y=cartCurrent] {\itersIPOPT}; 
\addlegendentry{Cart-Current}
\end{axis}

\end{tikzpicture}

==> figures/OPFvariantsItersIPOPTma57.tex <==
\begin{tikzpicture}

% COLORS 
%4-class OrRd Tokyo SIAM PP18
\definecolor{mycolor0}{HTML}{2B83BA}
\definecolor{mycolor1}{HTML}{D7301F}
\definecolor{mycolor2}{HTML}{FC8D59}
\definecolor{mycolor3}{HTML}{FDCC8A}
\definecolor{mycolor4}{HTML}{FEF0D9}
\definecolor{mycolor5}{HTML}{FEF0D9}
\definecolor{mycolor6}{HTML}{009933}

\pgfplotstableread{
id case polarPower cartPower polarCurrent cartCurrent 
1 1951rte 34  30  33  32
2 2383wp  47  46  46  45
3 2736sp  19  25  22  22
4 2737sop 23  22  18  21
5 2746wop 14  29  14  30
6 2746wp  16  29  16  27
7 2868rte 33  39  43  38
8 2869pegase  32  38  32  34
9 3012wp  42  40  39  40
10 3120sp  41  55  38  42
11 3375wp  42  39  42  40
12 6468rte 35  48  37  55
13 6470rte 50  50  43  55
14 6495rte 56  71  55  70
15 6515rte 54  64  55  62
16 9241pegase  47  51  42  46
17 ACTIVSg2000    24  33  26  31
18 ACTIVSg10k 30  32  32  36
19 13659pegase 66  62  67  70
20 ACTIVSg25k 46  47  41  50
21 ACTIVSg70k 57  66  55  65
22 case21k            270   270  270  270
23 case42k            270   270  270 270
24 case99k            270   270  270 270
25 case193k           270  270 270 270
}\itersIPOPT;
%NAN=270
%23 case42k            370 {} {} {}

\begin{axis}[
width=\columnwidth, height=5.5cm, 
ybar,
bar width=2pt, 
%ymode=log, 
%log origin=infty,
ymin=0,
ymax=250,
axis lines*=left, 
ymajorgrids, yminorgrids,
xtick=data,
xticklabels from table={\itersIPOPT}{case},
%xtick={1,2,3,4,5,6,7,89,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24,25},
%xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18},
enlarge x limits=0.05,
%xmin=0.5,
xmax=25,
%xticklabels={1, 2, 4, 8, 16, 32, 64, 128, 256},
xticklabel style={align=center, rotate=60, xshift=-0.8cm, yshift=0.2cm, anchor=north, font=\scriptsize},
ytick={0,50,100,150,200,250},
%yticklabels={$10^{-1}$, , , , , , , , $10^0$, , , , , , , , ,$10^1$},
yticklabel style={font=\scriptsize},
ylabel style={font=\scriptsize},
xlabel style={font=\scriptsize},
ylabel={No. of Iterations},
%xlabel={Benchmark},
legend style={at={(0.3,1.05)},fill=white,legend cell align=left,align=right,draw=white!85!black,font=\scriptsize,legend columns=2},
%restrict y to domain*=250, % Cut values off at 14
% visualization depends on=rawy\as\rawy, % Save the unclipped values
after end axis/.code={ % Draw line indicating break
        \draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.02) -- (rel axis cs:1,1.02);
    },
clip=false
]
\addplot[fill=mycolor0] table[x=id, y=polarPower] {\itersIPOPT};
\addlegendentry{Polar-Power}
\addplot[fill=mycolor1, postaction={pattern=north east lines}] table[x=id, y=cartPower] {\itersIPOPT}; 
\addlegendentry{Cart-Power}
\addplot[fill=mycolor6, postaction={pattern=north west lines}] table[x=id, y=polarCurrent] {\itersIPOPT}; 
\addlegendentry{Polar-Current}
\addplot[fill=mycolor3, postaction={pattern=crosshatch}] table[x=id, y=cartCurrent] {\itersIPOPT}; 
\addlegendentry{Cart-Current}
\end{axis}

\end{tikzpicture}
